Shocking Sgr B2(N1) with its own outflow: A new perspective on segregation between O- and N-bearing molecules

We want to investigate the influence of the powerful outflow driven by the hot core Sgr B2(N1) on the gas molecular inventory of the surrounding medium. We used the data taken as part of the 3 mm imaging spectral-line survey ReMoCA (Re-exploring Molecular Complexity with ALMA). Integrated intensity maps of SO and SiO emission reveal a bipolar structure with blue-shifted emission dominantly extending to the SE from the centre of the hot core and red-shifted emission to the NW. This is also prominently observed in emission of other S-bearing molecules and species that only contain N as a heavy element, including COMs, but also CH3OH, CH3CHO, HNCO, and NH2CHO. For a selection of COMs and simpler species, spectra were modelled under the assumption of LTE and population diagrams were derived at two positions, one in each outflow lobe. From this analysis, we obtained rotational temperatures, which are in a range of ~100-200K, and column densities. Abundances were subsequently compared to predictions of astrochemical models and to observations of L1157-B1, a position located in the well-studied outflow of the low-mass protostar L1157, and the source G+0.693-0.027, located in the Sgr B2 molecular cloud complex. Given the short distance of the analysed outflow positions to the centre of Sgr B2(N1), we propose a scenario in which a phase of hot-core chemistry (i.e. thermal desorption of ice species and high-temperature gas-phase chemistry) preceded a shock wave. The subsequent compression and further heating of the material resulted in the accelerated destruction of (mainly O-bearing) molecules. Gas-phase formation of cyanides seems to be able to compete with their destruction in the post-shock gas. Abundances of HCnN (n=3,5) are enhanced in the outflow component pointing to (additional) gas-phase formation. To confirm such a scenario, appropriate chemical shock models need to be run.

==> modelcf_backup.tex <==
\subsubsection{N1S and N1S1}\label{sss:n1s}

By assuming a slow warm-up (SWU) phase, abundances of the cyanides at N1S and N1S1 can be more less reproduced by the model, those of NH\2CN and \fmm are underestimated by factors of a few, those of \mic by about two orders of magnitude. The abundance of HNCO is slightly overproduced by the model for N1S, that of HC\3N by two orders of magnitude. Abundances of all O-bearing molecules are overestimated by the model by factors of a few up to an order of magnitude. Methyl mercaptan is underproduced by roughly a factor 10.
In contrast, for a fast warm-up (FWU), the abundance of HC\3N is better reproduced by the model, and those of methyl and vinyl cyanide are underestimated by a larger amount than for the SWU. The prediction for formamide is slightly worse. Observed abundances for \ad agree well with the prediction, those of \mf and \dme match better as well, and there are no significant changes seen for methanol and ethanol.
%In the model, their abundances were generally underestimated, which is also seen for position N1S in Fig.\,\ref{fig:cfmodel} for \vc, \etc, \fmm, and \mic. 
Abundances of most molecules at N1S and N1S1 have been derived in Paper\,I and compared to the G22 model (assuming SWU). The observed abundance profiles of N- and (N+O)-bearing COMs showed either a plateau or an increasing behaviour at temperatures above 100\,K. In particular, the increase of abundances at high temperatures pointed to the COMs' formation partly or solely in the gas phase at these temperatures. 
A more efficient conversion from HC\3N to \vc and, eventually, \etc on dust grain surfaces  was suggested as a possible way to increase the abundances of these cyanides, because they were found to be underestimated by the model in Paper\,I. Implementing this to the model may then also decrease the HC\3N abundance, which is currently overproduced by the SWU model for N1S. This could also apply to the FWU, however to a smaller extent, maybe due to the shorter timescale. 
Methyl cyanide was not analysed in Paper\,I, however, based on the value previously derived at N1S \citep{Mueller21} and those derived in this work for N1SE1 (cf. Fig.\,\ref{fig:Xbars-norm}), the COM's behaviour seems to be comparable to the other cyanides pointing the COM's formation in the gas phase. This is in agreement with the model that predicts efficient gas-phase formation of the molecule, mainly from the recombination of CH\3CNH$^+$ with an electron, where the protonated methyl cyanide is a product of the gas-phase reaction CH\3$^+$ + HCN.
If we assume a FWU, the CH\3CN production has to proceed more efficiently in the model or there exist one or more additional formation routes (likely in the gas phase) that are currently not considered in the model.
The abundance value of NH\2CN was taken from an earlier ReMoCA result for N1S \citep{Kisiel22}. % and is higher by almost two orders of magnitude in the observations than in the model. 
The molecule is predicted to be solely formed at earliest times during stage 1, that is when the ice mantles start to build. According to G22, a high observed abundance of this molecule suggests that photoprocessing of the ice mantles at these early times could have been significant. This formation at early times explains the little difference between SWU and FWU.

The peak abundances for most O-bearing COMs were found at positions further away from Sgr\,B2\,(N1) than N1S in Paper\,I. These peaks resulted from the COMs' thermal desorption at $\sim$100\,K and their subsequent destruction in the gas phase at higher temperatures, that is shorter distances to the centre of the hot core. This can explain why the observed abundances at N1S are lower than the model predictions. In the FWU, there was less time to destroy \dme and \mf, explaining the better agreement with the model. For \et we discussed in Paper\,I that additional grain-surface processes could potentially reduce the modelled peak abundances to better match the observed value (maybe in addition to a shorter destruction time period). 
Acetaldehyde is dominantly formed in the gas phase in the models. Therefore, the overproduction at N1S and N1S1 in the SWU models has to have another origin than for the other O-bearing species. Because the abundance is well reproduced for the FWU, maybe the heating timescale is the reason, which was also mentioned in Paper\,I.  %Therefore, the  model overproduces acetaldehyde at N1S1 by nearly a factor of 10. 
%This may result from the facts that the COM is a gas-phase product and N1S1 is further away from the centre of the hot core than N1S, which means that the gas-phase chemistry is less advanced.
The chemical network for \mic is incomplete, which is likely the main reason for the heavy underestimation of its abundances in all models that we compare to in Fig.\,\ref{fig:cfmodel}. Formamide is formed mainly on dust grains, but also in the gas phase to some extent, and it gets destroyed after thermal desorption in the gas phase. The abundance profiles derived in Paper\,I also suggested that both formation pathways could play a role in setting the COM's gas-phase abundance. However, there was no clear evidence for efficient destruction of the COM at high temperatures as predicted by the model. 
The abundance of HNCO was additionally computed in this work for N1S and seems to agree well with the modelled value. In the model, HNCO is a product of grain-surface chemistry and gets destroyed in the gas phase after desorption. 

Methyl mercaptan is a pure product of grain-surface chemistry and is formed mainly via H addition to CS during the collapse as well as the subsequent warm-up phase as can be seen from its panel in Fig.\,\ref{fig:G22}, which assumes a SWU. This kind of figure is an output of the G22 models and such plots were presented for a variety of molecules in Figs.\,13--14 in their article. These figures show qualitatively at what times (and temperature regime) of the pre- and protostellar evolution a molecule is dominantly formed (green) or destroyed (blue). The underestimation of \mmc abundances in the model may be the consequence of the fact that some input parameters related to sulphur chemistry are still uncertain in chemical models, for example the initial elemental abundance of S (G22) in general or, specifically for \mmc, the activation barriers for some of the reactions that eventually lead to the formation of the COM. 

\subsubsection{N1SE1}\label{dss:model_n1se1}

The comparison to N1S and N1S1 in Fig.\,\ref{fig:cfmodel} shows that the abundances with respect to H\2 of all O-bearing molecules are more underestimated in the model for N1SE1:HC, and even more for N1SE1:OF. The difference between the SWU and FWU are not significant, except for \ad, where again the FWU is a better match. Abundances of the cyanides behave similarly at all positions, that is, the predictions of the SWU better match the observed abundances. Only \vc is slightly more underproduced in the model in both components at N1SE1 than at N1S and N1S1 for both the SWU and FWU. Abundances of HC\3N are similarly overestimated by the SWU model for N1SE1:HC and OF by factors of a few and are both lower by a factor 10 than at N1S. In the FWU, HC\3N is underproduced in contrast to the results at N1S and in contrast to the results for N1SE1 for the SWU. The only secure detection of HC\5N was done in the outflow component at N1SE1 and its abundance is overestimated by the SWU model by two orders of magnitude while it is well reproduced assuming a FWU. The observed abundance of \mmc is more or less in agreement in both the SWU and FWU models at N1SE1:HC, while it is underestimated by factors of a few in the outflow component at N1SE1, similar to N1S. Abundances of OCS are underestimated by roughly two orders of magnitude in both N1SE1:HC and OF for the SWU, while they are slightly better reproduced by the FWU. 

A more efficient conversion of HC\3N to \vc and \etc in the solid phase as proposed in Sect.\,\ref{sss:n1s} may help to better match the modelled and observed HC\3N abundances for the SWU, however, it would lead to a larger discrepancy for the cyanides in this case and does not help at all the results for the FWU. 
The secure detection of HC\5N at N1SE1:OF may suggest that gas-phase chemistry plays an important role in this component. Not only this molecule but also HC\3N have both efficient formation pathways occurring at around 200\,K in the gas phase, where C\2H and HCN react to form HC\3N, which will again react with C\2H to form HC\5N. 
We show the rate of change for the SWU in HC\5N abundance in Fig.\,\ref{fig:G22}, where it is evident that the bulk of the molecule is produced in the gas phase at not only around 200\,K, but there is a second period of efficient production of the molecule at $\sim$350--400\,K. In addition to the reaction mentioned above, at these temperatures atomic N, which was sourced from NH\3 via H abstraction, reacts with hydrocarbons such as, for example C\5H\2, to form HC\5N. Our analysis did not reveal temperatures as high as 400\,K, however, if a shock passed through the gas at N1SE1, the temperature might have reached a higher value momentarily. 
If we assumed a FWU (to approach shock conditions), and an enhanced gas-phase chemistry triggered by this event, perhaps abundances of CH\3CN, \vc, HC\3N, and OCS would increase to better match the observed value, however, the difference between model and observations would increase for HC\5N and also \ad. This applies to both components at N1SE1.

%Then maybe, at this position, solid-phase production of cyanides does not contribute much (anymore) to their gas-phase abundances or gas-phase formation is enhanced or both. Given that all N-bearing molecules, except maybe NH\2CN, are dominantly or partly produced in the gas phase, according to the results found in Paper\,I or to the model or both, enhanced gas-phase formation could be a plausible mechanism for the observed enhancement of N-bearing molecules at N1SE1. 

%Given that observed abundances of N-bearing molecules (with respect to methanol) are enhanced in both components of N1SE1 compared to N1S, it is not surprising that the modelled abundances are even more underestimated. In the outflow component even HC\3N abundances are now higher than predicted by the model (see Fig.\,\ref{fig:cfmodel}). 


%\textit{(If HC\5N is this high-T gas-phase product, which reactions give us this molecule and C-chains in general in all the cold regions like TMC-1?)}
%cyanopolyynes are supposed to be mainly formed in the gas phase \citep[][and references therein]{Bianchi23} 
%Cyanamide is similarly underproduced at N1S and N1SE1 in the model. This may suggest that it is not a product of an enhanced gas-phase chemistry, which is also not a prediction of the model.

As already seen for N1S and N1S1, \mic abundances are heavily underestimated in the model by multiple orders of magnitude certainly at N1SE1:HC likely due to an incomplete chemical network in particular. In Paper\,I we discussed additional formation routes that could potentially increase abundances in the model, in which \mic is currently solely produced on dust grain surfaces. However, although the observed abundance profile derived in Paper\,I might hint towards (partial) gas-phase formation, the only reaction with reactants HNCO and CH\3 that was first proposed to be efficient \citep[][]{Halfen15,Martin-Domenech17,Quenard18}, may actually proceed endothermically  \citep[][]{Halfen15,Majumdar18}. In the potential post-shock gas at N1SE1:OF (also HC to some extent) these reactions may however be able to take place. However, this would still not explain the differences at N1S and N1S1.
Abundances of \fmm are underestimated in the model for N1S, N1S1, and N1SE1:HC, but it is overestimated for the outflow component for both the SWU and FWU. Although efficient destruction in the gas phase at high temperatures was predicted in the model, there was no clear evidence for that in the abundance profiles of \fmm in Paper\,I. Therefore, for example, we proposed that the destruction should perhaps be less efficient in the model in order to reduce the difference to the observations. %Then at N1SE1:OF, the destruction may be as efficient as predicted by the model, which may be supported by the abundance values relative to H\2 that can be lower by more than an order of magnitude compared to N1S (see Fig.\,\ref{fig:Xbars-norm}). 
Abundances of HNCO behave similar to those of \fmm at N1SE1, except that the over- or underproductions are not as severe. In the model, \fmm and HNCO are correlated in the sense that they are produced and destroyed at similar periods of time and temperatures. A difference is however that HNCO is purely formed on dust grain surfaces, but it can be a by-product of COM dissociation at higher temperatures in the gas-phase \citep{Garrod08,Tideswell08}. %Perhaps, additional gas-phase production of HNCO can increase the modelled abundance to better match the observed value. In Paper\,I, we were able to roughly connect the emission morphology of a COM to its main formation pathway, where those mainly formed on dust grains showed a more extended and structured morphology, while emission from molecules that are mainly formed in the gas phase was more compact. The emission morphology of HNCO shown in Fig.\,4 in Paper\,I is similar to those of, for example HC\3N or \vc, which may be supportive of (partial) gas-phase formation of HNCO, similar to these other two molecules. 

The overall larger overestimation of abundances of O-bearing molecules in the model suggests an enhanced destruction of these, specifically, COMs in N1SE1:HC and even more so in N1SE1:OF in the gas phase after their desorption from the dust grains. Again, this explanation does not apply to \ad as it is primarily a gas-phase product. Moreover, given that HNCO and NH\2CN are products of grain-surface chemistry and are efficiently destroyed in the gas phase in the model, we would expect them to behave more similarly to the O-bearing COMs. This suggests that there may be an additional reservoir of HNCO and NH\2CN (in the gas phase) or the destruction of the two proceeds less efficiently.  
In Paper\,I, we were able to roughly connect the emission morphology of a COM to its main formation pathway, where those mainly formed on dust grains showed a more extended and structured morphology, while emission from molecules that are mainly formed in the gas phase was more compact. The emission morphology of HNCO shown in Fig.\,4 in Paper\,I is similar to those of, for example HC\3N or \vc, which may be supportive of (partial) gas-phase formation of HNCO, similar to the two N-bearing molecules, perhaps due to the breakdown of COMs. %  between the model and the observations at N1S and N1SE1:HC are similar. Given that most O-bearing COMs are not detected in the outflow component, the question arises whether the outflow adds to the destruction of these molecules or they are not a product of an enhanced gas-phase chemistry as proposed for the N-bearing molecules. The comparison of abundances with respect to H\2 follows below. %at N1S and N1SE1:OF shows that O-bearing molecules are less abundant by up to an order of magnitude or more. This is also true for N1SE1:HC, but not as severely as for the outflow component. 

As mentioned before, the predictions for \mmc may have higher uncertainties due to unknowns in the sulphur chemistry in general and the chemistry of the COM in particular (see Sect.\,\ref{sss:n1s}). % are similarly underestimated in the model for N1S and N1SE1:HC, while the difference between model and observations is even larger for the outflow component. This may suggest that there exists another formation pathway, maybe in the gas phase, that we are currently not aware of.
The underestimation of the OCS abundances by the model is more severe. We show the rate of change for the SWU of the molecule's abundance during the protostellar evolution in Fig.\,\ref{fig:G22}. The molecule is mainly formed towards the end of the collapse phase, where the reaction S + CO produces OCS on the dust grain surfaces. In the current model, the activation barrier for this reaction is set to zero, while this assumption may not actually be correct \citep[][]{Loison12}. A non-zero activation barrier would however worsen the difference between the model and the observations. There  are a few reactions that produce OCS in the gas phase in the model. However, these are currently not able to reproduce the observed abundance. %: O + HCS $\rightarrow$ OCS + H (?). 
%At least one of these gas-phase reactions was found to have a substantial barrier that needs to be overcome \textit{(reference)}. Perhaps, physical conditions that are met in a post-shock gas could facilitate the occurrence of this reaction. %Figure\,\ref{fig:G22} also shows that OCS is efficiently destroyed, which results from its reaction with atomic H to form CO and HS.

%Based on Fig.\,\ref{fig:Xbars-norm}, we saw that abundances of \etc with respect to H\2 did not change significantly, therefore, we also compare the observations with the model in terms of abundances with respect to \etc in Fig.\,\ref{fig:cfmodelH2}. For N1S, the picture is not too different, while for N1SE1 it is, however. Abundances of HC\3N are overestimated, even more so those of HC\5N, while abundances of the other cyanides are comparable to the model predictions or slightly lower in the case of \vc. Abundances of O-bearing molecules are overproduced in the model for N1SE1:HC and even more for N1SE1:OF, perhaps suggesting an even more enhanced destruction of O-bearing molecules in the gas phase in the outflow component. Formamide and HNCO abundances show opposite behaviour in the outflow and hot-core components and \mic remains underproduced in the model at least in the hot-core component. 
%This comparison does not necessarily support a scenario of enhanced gas-phase formation traced by enhanced abundances of N-bearing molecules. It may rather suggest an enhanced destruction of O-bearing molecules in both the hot-core and outflow components at N1SE1 compared to N1S.
%Also, abundances of S-bearing species remain underestimated, however, less severely. 



Allen comparison
Based on the abundance profiles that we derived for Sgr\,B2\,(N1) in Paper\,I, we could see that abundances of \etc, but especially \vc, peak at high temperatures suggesting that they are (partly) formed in the gas phase. Therefore, it may not be surprising that abundances are higher for these species in the hotter sources B3 and A ($T>250$\,K) than in the colder sources B1 and B2 ($T<180$\,K). However, in B3 also O-bearing molecules are generally more abundant than in the other sources, or at least similarly abundant. Again, based on the abundance profiles in Paper\,I, according to which abundances of O-bearing molecules decreased towards higher temperatures, one would rather expect the colder sources to show higher abundances in these species, at least, compared to B3, given that similar sizes and masses for B1--B3 were reported \citep{Allen17}. However, the authors used average kinetic temperatures for their classification of the sources that they derived using CH\3CN. The actual range of temperatures shows that the sources could be more similar to each other. %Moreover, excitation temperatures that they derived in each source do not always show the same trend seen in kinetic temperatures. However, excitation temperatures for HC\3N and CH\3CN do not exceed 140\,K in sources B1 and B2, which is perhaps too cold for the production of \etc and \vc to an detectable amount, provided \etc indeed is a gas-phase product. 
\citet{Zhang22} reported on a spiral-like structure around B1 in SO\2 emission, which is associated with a disk and which also coincides with the continuum peaks B3 and B2. In addition, sources A and B1 drive outflows \citep[e.g.][]{Zhang22} and there is also SiO emission associated with the filament in which all sources are embedded. Therefore, one or more sources could be impacted by shocks. For example, this may have heated up B3, which enabled the production of N-bearing species. 
